Residual-Based Detection of Attacks in Cyber-Physical Inverter-Based Microgrids

This paper discusses the challenges faced by cyber-physical microgrids (MGs) due to the inclusion of information and communication technologies in their already complex, multi-layered systems. The work identifies a research gap in modeling and analyzing stealthy intermittent integrity attacks in MGs, which are designed to maximize damage and cancel secondary control objectives. To address this, the paper proposes a nonlinear residual-based observer approach to detect and mitigate such attacks. In order to ensure a stable operation of the MG, the formulation then incorporates stability constraints along with the detection observer. The proposed design is validated through case studies on a MG benchmark with four distributed generators, demonstrating its effectiveness in detecting attacks while satisfying network and stability constraints.

==> 0-nomenclature.tex <==
\vspace{-3mm}
\section*{Nomenclature}
\vspace{-2mm}
%
% list of used symbols, with their definition
\begin{itemize}
    \item $v_{bi}$: 3$\varphi$ voltage measured after the output connector\\ ($v_{bdi}$, $v_{bqi}$: $d$-  and $q$- axis component at $i_{th}$ inverter).
    \item $v_{oi}$: 3$\varphi$ voltage measured after the LC filter\\ ($v_{odi}$, $v_{oqi}$: $d$- and $q$- axis component at the $i_{th}$ inverter).
    \item $i_{oi}$: 3$\varphi$ current measured after the LC filter\\ ($i_{odi}$, $i_{oqi}$: d- and q- axis component at the $i_{th}$ inverter).
    \item $i_{li}$: 3$\varphi$ current measured before the LC filter\\ ($i_{ldi}$, $i_{lqi}$: $d$- and $q$- axis component at the $i_{th}$ inverter).
    \item $|v_{o}|$: voltage magnitude at the $i_{th}$ inverter.
    %\item $v_{odi}$ Voltage measured after the LC Filter in terms of d axis component at the $i_{th}$ DG.
    %\item $v_{oqi}$ Voltage measured after the LC Filter in terms of q axis component at the $i_{th}$ DG.
    %\item PI Proportional-Integral.
    \item $\delta_{i}$: rotating angle of the $i_{th}$ inverter.
    \item $\omega_i$: frequency at the $i_{th}$ inverter.
    \item $\omega_{ni}$: output of the secondary controller for frequency at the $i_{th}$ inverter.
    \item {$\omega_{ref}$: reference frequency value for the secondary controller.}
    \item $\omega_{ci}$: cut-off frequency of the low pass filter for the active and reactive power at the $i_{th}$ inverter.
    \item $\omega_{b}$: nominal angular frequency of the MG.
    \item $\omega_{com}$: Frequency of the common reference frame.
    \item $P_{i}$: active power of the $i_{th}$ inverter.
    \item $Q_{i}$: reactive power of the $i_{th}$ inverter.
    \item $V_{ni}$: output of the secondary controller for voltage at the $i_{th}$ inverter.
    %\item $v^*_{o}$: reference value for the output voltage magnitude at the $i_{th}$ DG.
    \item {$v_{ref}$: reference voltage value for the secondary controller}
    %\item $v^*_{odi}$ Reference value for the output voltage magnitude in terms of d axis component at the $i_{th}$ DG.
    %\item $v^*_{oqi}$ Reference value for the output voltage magnitude in terms of q axis component at the $i_{th}$ DG.
    \item $m_{Pi}$: Active droop coefficient at the $i_{th}$ inverter.
    \item $n_{Qi}$: Reactive droop coefficient at the $i_{th}$ inverter.
    %\item $\phi_{di}$ Auxiliary state variable in terms of d axis component at the $i_{th}$ DG. 
    %\item $\phi_{qi}$ Auxiliary state variable in terms of q axis component at the $i_{th}$ DG. 
    %\item $K_{PVi}$ Proportional Constant of the PI block located at the Voltage Controller.
    %\item $K_{IVi}$ Integral Constant of the PI block located at the Voltage Controller.
    \item $F_{i}$ current compensator at the $i_{th}$ DG.
    %\item $i^*_{1di}$ Output of the Voltage Controller in terms of d axis component at the $i_{th}$ DG.
    %\item $i^*_{1qi}$ Output of the Voltage Controller in terms of q axis component at the $i_{th}$ DG.
    %\item $\gamma_{di}$ Auxiliary state variable in terms of d axis component at the $i_{th}$ DG. 
    %\item $\gamma_{qi}$ Auxiliary state variable in terms of q axis component at the $i_{th}$ DG.
    %\item $K_{PCi}$ Proportional Constant of the PI block located at the Current Controller.
    %\item $K_{ICi}$ Integral Constant of the PI block located at the Current Controller.
    %\item $v^*_{idi}$ Output of the Current Controller in terms of d axis component at the $i_{th}$ DG.
    %\item $v^*_{iqi}$ Output of the Current Controller in terms of q axis component at the $i_{th}$ DG.
    \item $Z_{f}$: value of the impedance at the LC filter.
    %\item $R_{f}$: value of resistance located at the LC filter (VCVSI).
    %\item $L_{f}$: value of inductance located at the LC filter (VCVSI).
    %\item $C_{f}$: value of capacitance located at the LC filter (VCVSI).
    \item $Z_{f}$: value of the impedance at the output connector.
    %\item $R_{c}$: value of resistance at output connector (VCVSI).
    %\item $L_{c}$: value of inductance at output connector (VCVSI).
\end{itemize}

==> misc.tex <==







\section{Simulation Results}

\iffalse
\begin{table}[t]
\captionsetup{font=small}
\centering
\caption{Parameters of the test MG.}
\begin{tabular}{||c|c||c|c||} 
\hline \hline
\multicolumn{2}{||c||}{DGs 1 \& 2~}     & \multicolumn{2}{c||}{DGs 3 \& 4}      \\ 
\hline \hline
Parameter & Value & Parameter & Value \\
\hline \hline
$m_{P}$  & 9.4 x 10\textsuperscript{-5} & $m_{P}$  & 12.5 x 10\textsuperscript{-5}  \\ 
\hline
$n_{Q}$  & 1.3 x 10\textsuperscript{-3}  & $n_{Q}$  & 1.5 x 10\textsuperscript{-3}   \\ 
\hline
$R_{c}$  & 0.03 $\Omega$                         & $R_{c}$  & 0.03 $\Omega$                         \\ 
\hline
$L_{c}$  & 0.35 mH                       & $L_{c}$  & 0.35 mH                      \\ 
\hline
$R_{f}$  & 0.1 $\Omega$                           & $R_{f}$  & 0.1 $\Omega$                          \\ 
\hline
$L_{f}$  & 1.35 mH                       & $L_{f}$  & 1.35 mH                      \\ 
\hline
$C_{f}$  & 50 $\mu$F                         & $C_{f}$  & 50 $\mu$F                        \\ 
\hline
$K_{PV}$ & 0.1                           & $K_{PV}$ & 0.05                         \\ 
\hline
$K_{IV}$ & 420                           & $K_{IV}$ & 390                          \\ 
\hline
$K_{PC}$ & 15                            & $K_{PC}$ & 10.5                         \\ 
\hline
$K_{IC}$ & 20000                         & $K_{IC}$ & 16000                        \\ 
\hline
$\omega_{b}$  & 314.16 rad/s                       & $\omega_{b}$  & 314.16 rad/s                      \\ 
\hline
$F$   & 0.75                          & $F$   & 0.75                         \\ 
\hline
$\omega_{c}$  & 31.41 Hz                        & $\omega_{c}$  & 31.41 Hz                        \\
\hline
$c_{f}$  & 30                         & $c_{f}$  & 30                        \\
\hline
$c_{v}$  & 30                         & $c_{v}$  & 30                        \\
\hline \hline
\end{tabular}
\label{table_I}
\end{table}
%
%
\begin{table}[t]
\captionsetup{font=small}
\centering
\caption{Parameters of lines and loads.}
\begin{tabular}{||c|c|c|c|c|c|c|c||} 
\hline \hline
\multicolumn{4}{||c|}{Lines 1, 3}                             & \multicolumn{4}{c||}{Line 2}                                 \\ 
\hline \hline
\multicolumn{2}{||c|}{$R_{line}$}    & \multicolumn{2}{c|}{0.23 $\Omega$}   & \multicolumn{2}{c|}{$R_{line}$}  & \multicolumn{2}{c||}{0.35 $\Omega$}     \\ 
\hline
\multicolumn{2}{||c|}{$L_{line}$}    & \multicolumn{2}{c|}{318 $\mu$H} & \multicolumn{2}{c|}{$L_{line}$}  & \multicolumn{2}{c||}{1847 $\mu$H}  \\ 
\hline
\multicolumn{2}{||c|}{Load 1}   & \multicolumn{2}{c|}{Load 2} & \multicolumn{2}{c|}{Load 3} & \multicolumn{2}{c||}{Load 4}   \\ 
\hline
R & 30 $\Omega$                         & R & 20 $\Omega$                      & R & 25 $\Omega$                      & R & 25 $\Omega$                        \\ 
\hline
X & 15 $\Omega$                         & X & 10 $\Omega$                      & X & 10 $\Omega$                     & X & 15 $\Omega$                       \\
\hline \hline
\end{tabular}
\label{table_II}
\end{table}

\begin{figure}[t]
    \centering
        \includegraphics[width=0.45\textwidth]{Figures_Paper/No_attack_DG1_DG4.pdf}
    \caption{Attack-free scenario.}
    \label{no_attack}
\end{figure}
\fi 

\begin{table}[t]
\captionsetup{font=small}
\caption{Modeling Scenarios against DG 1 and DG 4.}
\vspace{-1mm}
\begin{center}
\begin{tabular}{||c|c|c|c||} 
 \hline \hline  
 % &&&&\\
Attack&Modeling&Voltage&Frequency\\
 %Ratio&(\%)&(\%)&(\%)&(\%)\\
Scenario&  & Values & Values \\
 %&$k = 10$&$k = 40$&$k = 80$&$k = 130$\\
 \hline
 \hline
 Eqs. \eqref{eq:fdia-omega},\eqref{eq:fdia-voltage} &Uniform Distribution&$\mu[-0.2, 0.2]$&$\mu[-5,5]$\\
 \hline 
 Eqs. \eqref{eq:jamming-omega},\eqref{eq:jamming-voltage} &Normal Distribution&$\mathcal{N}(0, 0.2)$&$\mathcal{N}(0, 5)$\\
 \hline
 Eqs. \eqref{eq:hybrid-omega},\eqref{eq:hybrid-voltage} &Uniform + Normal&$\mu$ + $\mathcal{N}$&$\mu$ + $\mathcal{N}$\\ 
 \hline
 Eqs. \eqref{eq:dos-omega},\eqref{eq:dos-voltage} &Additive Inverse&-- $V_{ni}$& -- $\omega_{ni}$\\ 
 \hline
 Eqs. \eqref{eq:sinusoidal-omega},\eqref{eq:sinusoidal-voltage} & Sine Function & $0.3*sin(t)$ & $20*sin(t)$\\ 
 \hline \hline  
 \end{tabular}
\end{center}
\label{table_III}
\end{table}



Below, the different attack signals investigated in this paper (i.e., $\omega_{a}$ and $V_{a}$ %in \eqref{secondary_att}) 
are modeled:
\vspace{-2mm}
\begin{subequations}
    \label{eq:omega-attack}
    \begin{align}
    & \omega_{a_{1}} = \mu[-\lambda_{{min}},\lambda_{{max}}] \label{eq:fdia-omega}\\
    & \omega_{a_{2}} = \mathcal{N}(\mu_\nu,\,\sigma^2_\nu) \label{eq:jamming-omega} \\
    & \omega_{a_{3}} = \gamma \label{eq:hybrid-omega} \\
    & \omega_{a_{4}} = - \omega_{ni} \label{eq:dos-omega} \\
    & \omega_{a_{5}} = A*sin(t) \label{eq:sinusoidal-omega}
    \end{align}
\end{subequations} \vspace{-5mm}
\begin{subequations}
    \label{eq:voltage-attack}
    \begin{align}
    & V_{a_{1}} = \mu[-\psi_{{min}},\psi_{{max}}] \label{eq:fdia-voltage}\\
    & V_{a_{2}} = \mathcal{N}(\mu_u,\,\sigma^2_u) \label{eq:jamming-voltage} \\
    & V_{a_{3}} = \kappa \label{eq:hybrid-voltage} \\
    & V_{a_{4}} = - V_{ni} \label{eq:dos-voltage} \\
    & V_{a_{5}} = B*sin(t) \label{eq:sinusoidal-voltage}
    \end{align}
\end{subequations}

\noindent where $\mu$ is described as a uniformly distributed random variable which makes the duplet $[\omega_{a_{1}},  V_{a_{1}}]$ to be seen as FDIA. $\mathcal{N}(\mu_\nu,\,\sigma^2_\nu)$ and $\mathcal{N}(\mu_u,\,\sigma^2_u)$ represent  normally distributed random variables that leads to the jamming attack representation of $[\omega_{a_{2}},  V_{a_{2}}]$.  $\beta$ and $\kappa$ can be seen as a hybrid-type of attack formulated as the superimposition of $\mu[-\lambda_{{min}},\lambda_{{max}}]$ to $\mathcal{N}(\mu_\nu,\,\sigma^2_\nu)$, and $\mu[-\psi_{{min}},\psi_{{max}}]$ to $\mathcal{N}(\mu_u,\,\sigma^2_u)$, respectively. Finally, $[\omega_{a_{4}},  V_{a_{4}}]$ represent a strategy in which the secondary controller output resembles a denial-of-service (DoS) attack that does not provide availability of the control signal, while $[\omega_{a_{5}},  V_{a_{5}}]$ is an additive attack of a sinusoidal signal with random amplitude. 


%
In this Section, the simulations results 
are presented demonstrating the impact of the cyber-attacks discussed in Section \ref{s:attackformulation}, and the effectiveness of the proposed detection and mitigation strategy of Section \ref{s:methodology}. The MG adopted for testing is shown in Fig.  \ref{fig1a}, and the relevant MG modeling parameters are detailed in Table \ref{table_I} and Table \ref{table_II}. 
\textcolor{blue}{The initial state of the observer is set equal to the measured state at the initial time.}
Simulation results have been performed with MATLAB 2020.b, on a Macbook Pro 2021, with 16 GB of RAM and a 512 GB hard disk drive. The source files, models, and code of the simulations associated with this work can be found online \cite{githubcode}. % 
%\href{https://github.com/aintriagov/Grid-Forming-Inverters-under-Cyber-Attacks.git}{this link}.


\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.315\textwidth]{Figures_Paper/FDI_DG1.pdf}
        \label{fig:FDI_attack_DG1}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\textwidth]{Figures_Paper/FDI_DG2.pdf}
        \label{fig:FDI_attack_DG2}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/Jamming_DG3.pdf}
        \label{fig:jamming_attack_DG3}
    } \\
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/Jamming_DG4.pdf}
        \label{fig:jamming_attack_DG4}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/DoS_attack.pdf}
        \label{fig:DoS_attack}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/Sinusoidal_Attack.pdf}
        \label{fig:sinusoidal_attack}
    } \\
    
\caption[CR]{Effects of the attack scenarios at the outputs of the secondary controller: (\subref{fig:FDI_attack_DG1}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage} against DG 1, (\subref{fig:FDI_attack_DG2}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage} against DG 1 and impact demonstrated on DG 2, (\subref{fig:jamming_attack_DG3}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage} against DGs 1 and 4, and impact demonstrated on DG 3, (\subref{fig:jamming_attack_DG4}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage} attack against DG 4, (\subref{fig:DoS_attack}) Eqs. \eqref{eq:dos-omega}, \eqref{eq:dos-voltage} attack against DGs 1 to 4, (\subref{fig:sinusoidal_attack}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage} attack against DGs 1 to 4.} 
\vspace{-3mm}
\label{fig:attacks}
\end{figure*}


% \begin{figure*}[t]
% \centering
%     \subfloat[]{
%         \includegraphics[width=0.4\textwidth]{Figures_Paper/FDI_DG2.pdf}
%         \label{fig:FDI_attack_DG2}
%     } 
%     \subfloat[]{
%         \includegraphics[width=0.4\linewidth]{Figures_Paper/FDI_DG3.pdf}
%         \label{fig:FDI_attack_DG3}
%     } \\
%     \subfloat[]{
%         \includegraphics[width=0.4\linewidth]{Figures_Paper/Jamming_DG2.pdf}
%         \label{fig:Jamming_attack_DG2}
%     } 
%     \subfloat[]{
%         \includegraphics[width=0.4\linewidth]{Figures_Paper/Jamming_DG3.pdf}
%         \label{fig:Jamming_attack_DG3}
%     } \\
    
% \caption[CR]{Effects of the attack scenarios at the outputs of the secondary controller: (\subref{fig:FDI_attack_DG2}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage} against DG 2, (\subref{fig:FDI_attack_DG3}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage} attack against DG 3, (\subref{fig:Jamming_attack_DG2}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage} attack against DG 2, (\subref{fig:Jamming_attack_DG3}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage} attack against DG 3.} 
% \vspace{-3mm}
% \label{fig:attacks}
% \end{figure*}










%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Impact of Attacks on VCVSI Output}
 
Fig. \ref{no_attack} displays the voltage and frequency values in the attack-free scenario. The reference values are set to $1$ per unit (p.u.) and $50$ Hz, respectively. The figure shows that the secondary controller works properly, i.e., voltage and frequency values reach the reference values. {The magnitudes of voltage and frequency in the DGs present instabilities after cyber-attacks are introduced into the system. This effect is produced by tampering the references provided by the secondary controller. This action leads to distorting the active and reactive power values of the generators inside the MG.}   

Attacks are being simulated on the output of the secondary controllers (i.e., signals $V_{ni}$ and $\omega_{ni}$ outlined in Section \ref{s:attackformulation}) of DGs 1 and 4. The attack duration is assumed to be bounded and last from $0.4s$ to $0.8s$.  As simulations demonstrate, the attacks impact along the MG, even though {DGs 2 and 3} 
do not have any signal directly corrupted. This behavior is reasonable as the DGs are interconnected via a physical layer and a communication network. The plots presented are only for specific DGs for brevity. The simulations results show both the behavior of a particular DG with a direct corruption of signals and a DG that is not under attack. These experiments exhibit that DGs \{2,3\} as well as DGs \{1,4\}  show similar behavior. 



%\hl{While attacking the outputs of the secondary controller, the references for the voltage and frequency will be displaced randomly, depending on the attack we are executing. Therefore, those quantities will oscillate regarding the values we inject into the secondary controller diagram. A little observation here is that even though the nominal values for frequency and voltage are being altered, the controller of the GFMI is robust until some point because it maintains those quantities in a specific interval.} 

Table \ref{table_III} shows the mathematical models behind the attacks introduced at DG 1 and 4. The voltage and frequency values were selected considering the acceptable range for voltage and frequency fluctuation of $v_{omagi}$ and $\omega_{i}$. These intervals go from $0.9$ to $1.1$ p.u. and $47.5$ to $51.5$ Hz  for voltage and frequency, respectively. In order to synthetically  generate such output ranges, the attack scenarios are considered under extreme conditions. The five case scenarios and their modeling aspects considered to attack the output of the secondary controller for voltage and frequency are provided in Table \ref{table_III}. {The goal of the threat actor is to collapse the MG operating state. Hence, voltage, frequency, and power will be subject to instabilities, leading to low performance of the power dispatch,  equipment damage, or potential system collapse.} 
 %To show the gravity of these scenarios, we have modeled five case studies where the voltage and frequency references are being altered. 

Fig. \ref{fig:FDI_attack_DG1} shows the impact of an attack modeled as in Eqs. \eqref{eq:fdia-omega} and \eqref{eq:fdia-voltage} {against the outputs of the secondary controllers of DG 1.  The attack function aims to compromise the voltage reference. The same approach is used for the frequency. Fig. \ref{fig:FDI_attack_DG2} shows how DG 2 responds in such attack vector introduced into its neighbors agents (DG 1).} 
Fig. \ref{fig:jamming_attack_DG3} and \ref{fig:jamming_attack_DG4} present the impact of an attack modeled as in Eqs. \eqref{eq:jamming-omega} and \eqref{eq:jamming-voltage}, against DGs 1 and 4. The attack vector is intended to affect the system's voltage and frequency stability while tampering the pre-defined setpoints of the MG. {Even though DGs 2 3 are not being directly corrupted,  Fig. \ref{fig:jamming_attack_DG3} depicts a (slight) variation in the magnitudes of voltage and frequency.} 
The hybrid attack modeled in Eqs. \eqref{eq:hybrid-omega} and \eqref{eq:hybrid-voltage} has a similar impact as the one depicted in Fig. \ref{fig:jamming_attack_DG4}, and the related simulation is not reported for brevity, but can be found in the simulation data provided and associated with this work in \cite{githubcode}. Fig.~\ref{fig:DoS_attack} shows the effects of these attacks, modeled by \eqref{eq:dos-omega} and \eqref{eq:dos-voltage}. Here, simulations show how the DoS affects the four DGs. The voltage and frequency values for DGs 1 and 4 have faster decay than DGs 2 and 3. This behavior is reasonable because the reference values for DGs 1 and 4 are set to zero. At the same time, for DGs 2 and 3, the decay is different because the MG has been designed as a multi-agent system where each agent exchanges information with its neighbors. 
 This scenario implies the interruption of the communication of the voltage and frequency references provided by the secondary controller. The voltage and frequency signals eventually go to zero when the references are the same, demonstrating the severe impact of such scenario in terms of not serving load. %This attack is considered one of the most dangerous since it can cause a power outage and affect consumers. 
%This case scenario shows us explicitly that a threat actor has compromised our system by finding an entry point to execute vulnerabilities. 
Finally, Fig. \ref{fig:sinusoidal_attack} depicts the impact of a sinusoidal additive attack in the MG, described by \eqref{eq:sinusoidal-omega} and \eqref{eq:sinusoidal-voltage}.  

%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%


\iffalse
\subsection{Random attack vector on the communication links of the VCVSI}

\hl{HERE WRITE ABOUT THE SEVERAL RANDOM VECTORS USED WHILE TARGETING THE INPUTS OF THE GRID FORMING INVERTER}


\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.315\textwidth]{Figures_Paper/volt_freq_FDI_DG4_inputs.pdf}
        \label{fig:FDI_attack_DG4_INPUTS}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\textwidth]{Figures_Paper/volt_freq_jamming_DG4_inputs.pdf}
        \label{fig:JAMMING_attack_DG4_INPUTS}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/volt_freq_sinusoidal_normal_DG4_inputs.pdf}
        \label{fig:SINUSOIDAL_attack_DG4_INPUTS}
    } \\
   
    
\caption[CR]{Effects of the attack scenarios at the output of the DG 4: (\subref{fig:FDI_attack_DG4_INPUTS}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage}, (\subref{fig:JAMMING_attack_DG4_INPUTS}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage}, (\subref{fig:SINUSOIDAL_attack_DG4_INPUTS}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage}} 
\vspace{-3mm}
\label{fig:attacks_inputs}
\end{figure*}



\subsection{Stealthy and Intermittent Integrity attack vectors on the communication links of the VCVSI}

\hl{STEALTHY AND INTERMITTENT ATTACK VECTORS}
\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.23\textwidth]{Figures_Paper/attack_signal_au_b_0.2.pdf}
        \label{fig:stealthy_attack_au_b_0.2}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\textwidth]{Figures_Paper/input_signal_attack_a_b_0.2.pdf}
        \label{fig:stealthy_attack_a_b_0.2}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/stealthy_vomag_DG4_b_0.2.pdf}
        \label{fig:stealthy_attack_voltage_b_0.2}
    } 
   \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/stealthy_frequency_DG4_b_0.2.pdf}
        \label{fig:stealthy_attack_frequency_b_0.2}
    } \\

    \subfloat[]{
        \includegraphics[width=0.23\textwidth]{Figures_Paper/attack_signal_au_b_0.2.pdf}
        \label{fig:stealthy_attack_au_b_0.3}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\textwidth]{Figures_Paper/input_signal_attack_a_b_03.pdf}
        \label{fig:stealthy_attack_a_b_0.3}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/stealthy_vomag_DG4_03.pdf}
        \label{fig:stealthy_attack_voltage_b_0.3}
    } 
   \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/stealthy_frequency_DG4_03.pdf}
        \label{fig:stealthy_attack_frequency_b_0.3}
    } \\
    
\caption[CR]{Effects of the stealthy attack at the outputs of DG 4 with different b values: (\subref{fig:FDI_attack_DG4_INPUTS}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage}, (\subref{fig:JAMMING_attack_DG4_INPUTS}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage}, (\subref{fig:SINUSOIDAL_attack_DG4_INPUTS}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage}} 
\vspace{-3mm}
\label{fig: stealthy_attack_input}
\end{figure*}


\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.23\textwidth]{Figures_Paper/attack_intermittent_input_au_b_02.pdf}
        \label{fig:stealthy_intermittent_attack_au_b_0.2}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\textwidth]{Figures_Paper/intermittent_attack_beta_a_b_02.pdf}
        \label{fig:stealthy_intermittent_attack_a_b_0.2}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/stealthy_intermittent_vomag_DG4_02.pdf}
        \label{fig:stealthy_intermittent_attack_voltage_b_0.2}
    } 
   \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/stealthy_intermittent_frequency_DG4_02.pdf}
        \label{fig:stealthy_intermittent_attack_frequency_b_0.2}
    } \\
    \subfloat[]{
        \includegraphics[width=0.23\textwidth]{Figures_Paper/attack_intermittent_input_au_b_02.pdf}
        \label{fig:stealthy_intermittent_attack_au_b_0.3}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\textwidth]{Figures_Paper/intermittent_attack_beta_a_b_03.pdf}
        \label{fig:stealthy_intermittent_attack_a_b_0.3}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/stealthy_intermittent_vomag_DG4_03.pdf}
        \label{fig:stealthy_intermittent_attack_voltage_b_0.3}
    } 
   \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/stealthy_intermittent_frequency_DG4_03.pdf}
        \label{fig:stealthy_intermittent_attack_frequency_b_0.3}
    } \\
\caption[CR]{Effects of the stealthy intermittent integrity attack at the outputs of DG 4: (\subref{fig:FDI_attack_DG4_INPUTS}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage}, (\subref{fig:JAMMING_attack_DG4_INPUTS}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage}, (\subref{fig:SINUSOIDAL_attack_DG4_INPUTS}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage}} 
\vspace{-3mm}
\label{fig: stealthy_intermittent_integrity_attack_input}
\end{figure*}

\fi

\subsection{Euclidean norm of the residual}
The importance of observers relies on computing an error, described as the observer state error variable $\xi$, presented in Theorem 1. This error indicates that the MG is experimenting an anomalous behavior. The norm of the error vector, e.g., the Euclidean ${l}^2$ norm (i.e., $||\xi||_2  \triangleq  \sqrt{\sum_{i}\xi_i^2}$), can be computed to measure the error. The error acts as an alarm for this work's residual-based detection approach.  This paper focuses on effectively detecting attacks, and leverages a residual-threshold based approach. Similar to \cite{pajic2016attack}, where corrupted system states could be recovered with a 0.1 detection threshold, this proposed methodology is able to correctly identify corrupted values with a similar empirically-selected maximum error threshold. Fig. \ref{fig:l2norm} depicts the response of the residual norms without any mitigation strategy when the attack scenarios occur at the output of the secondary controller for voltage and frequency. From Fig. \ref{fig:FDI_L2norm} to Fig. \ref{fig:sinusoidal_L2norm}, it can be observed that the DGs behavior is sensitive to these perturbations, specially to the sinusoidal scenario, where the error diverges more critically, compared to the other residuals, produced by the attacks. 

\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.315\textwidth]{Figures_Paper/L2norm_FDI_DG1_DG4.pdf}
        \label{fig:FDI_L2norm}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/L2norm_Jamming_DG1_DG4.pdf}
        \label{fig:Jamming_L2norm}
    } 
    % \subfloat[]{
    %     \includegraphics[width=0.2\linewidth]{Figures_Paper/L2norm_Sinusoidal_DG1_DG4.pdf}
    %     \label{fig:control1}
    % } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/L2norm_Sinusoidal_DG1_DG4.pdf}
        \label{fig:sinusoidal_L2norm}
    } \\
    
\caption[CR]{${l}^2$ norm of the residual under attacks: (\subref{fig:FDI_L2norm}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage} attack targeting DGs 1 and 4, (\subref{fig:Jamming_L2norm}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage} attack targeting DGs 1 and 4, (\subref{fig:sinusoidal_L2norm}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage} attack targeting DGs 1 and 4.} 
%\vspace{-2mm}
\label{fig:l2norm}
\end{figure*}


\iffalse
\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.315\textwidth]{Figures_Paper/Residual_FDI_DG4_inputs.pdf}
        \label{fig:residual_FDI_inputs_DG4}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\textwidth]{Figures_Paper/residual_error_jamming_DG4.pdf}
        \label{fig:residual_Jamming_inputs_DG4}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/residual_error_sinusoidal_normal_DG4.pdf}
        \label{fig:residual_sinusoidal_normal_inputs_DG4}
    } \\
   
    
\caption[CR]{${l}^2$ norm of the residual under random attacks at the control signals of the VCVSI: (\subref{fig:residual_FDI_inputs_DG4}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage}, (\subref{fig:residual_Jamming_inputs_DG4}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage}, (\subref{fig:residual_sinusoidal_normal_inputs_DG4}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage}} 
\vspace{-3mm}
\label{fig:residual_random_attack_vector}
\end{figure*}



\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/residual_stealthy_DG4_b_0.2.pdf}
        \label{fig:residual_stealthy_0.2}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/residual_stealthy_DG4_03.pdf}
        \label{fig:residual_stealthy_0.3}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/residual_stealthy_intermittent_DG4_02.pdf}
        \label{fig:residual_stealthy_intermittent_0.2}
    } 
   \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/residual_stealthy_intermittent_DG4_03.pdf}
        \label{fig:residual_stealthy_intermittent_0.3}
    } \\
    
\caption[CR]{${l}^2$ norm of the residual of DG4 under a stealthy and intermittent attack vector with different b values: (\subref{fig:FDI_attack_DG4_INPUTS}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage}, (\subref{fig:JAMMING_attack_DG4_INPUTS}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage}, (\subref{fig:SINUSOIDAL_attack_DG4_INPUTS}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage}} 
\vspace{-3mm}
\label{fig: residuals_inputs_stealthy_attack_vector}
\end{figure*}
\fi





% \ref{fig:FDI_L2norm} \hl{shows the ${l}^2$ norm of the residual vector $\xi$ at DG 1 and DG 4, under the FDIA scenario. The ${l}^2$ norm is defined as $||\xi||_2  \triangleq  \sqrt{\sum_{i}\xi_i^2}$. The residual is initially different from zero since the initial state of the observer (set to $0.1$ for all the variables) is different from the state of the DG. After about $0.2s$, and until the attack is launched, at $0.4s$, the residual is approximately zero, which confirms that the proposed observer works correctly. At $0.4s$ when the attack is activated, a variation in the value of the norm of the residual is observed. The magnitude of the norm will depend on how prominent the aggression will be in the MG. 
% In the beginning, the system starts at zero, while the observer's state starts at $0.1s$. As can be noticed, DG 1 shows higher values than DG 4. This difference lies in the fact that the first DG has been set up as the leader node, which means its performance occurs first. Eventually, it will have to deal first with corrupted values located at the output of the secondary controller from frequency and voltage, which will affect its stable reference. DG 4, on the other side, will start acting after DG 1, which gives it time to reduce the impact of the cyber-attack.  
% The plots of the ${l}^2$ norm of the residual under the jamming} \ref{fig:Jamming_L2norm} and the hybrid attacks are similar to Fig. \ref{fig:FDI_L2norm}. 
% The DoS attack has the same behavior as Fig. \ref{fig:sinusoidal_L2norm} \hl{and is not reported for brevity. Compared to the FDI attacks, the DoS attack implies the interruption of the communication of the voltage and frequency references provided by the secondary controller. For these two attacks, the ${l}^2$ norm of one or both the residuals diverges, meaning that the attack makes the observer dynamics unstable, causing the estimation error to diverge.
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mitigation Strategy}
In this subsection, the  detection and mitigation strategy proposed in Section \ref{s:methodology} is applied to deal with the five attack scenarios analysed in Section \ref{s:attackformulation}. A threshold value is used as an alarm in case the DG inverter is experiencing abnormal operating values for frequency and voltage. In Figs.~\ref{fig:FDI_mitigation} to \ref{fig:sinusoidal_mitigation}, the attacks are neutralized, shielding each DG output voltage and frequencies. 
The detection and mitigation approach adopted is residual-based; in the time instants when one or more components of the  residual go beyond the respective threshold $\tau_i$, the DG controllers will use the estimated state values from the observer, instead of the measured values that triggered the residual-based detection condition. Consequently, protection of the MG is effectively guaranteed.

\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.32\textwidth]{Figures_Paper/Mitigation_FDI.pdf}
        \label{fig:FDI_mitigation}
    } 
    \subfloat[]{
        \includegraphics[width=0.32\linewidth]{Figures_Paper/Jamming_Mitigation.pdf}
        \label{fig:jamming_mitigation}
    } 
    \subfloat[]{
        \includegraphics[width=0.32\linewidth]{Figures_Paper/Sinusoidal_Mitigation.pdf}
        \label{fig:sinusoidal_mitigation}
    } \\ 
    
\caption[CR]{Detection and mitigation strategy applied at the DGs: (\subref{fig:FDI_mitigation}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage} attack against DGs 1 and 4, (\subref{fig:jamming_mitigation}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage} attack against DGs 1 and 4, (\subref{fig:sinusoidal_mitigation}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage} attack against DGs 1 and 4.} 
%\vspace{-2mm}
\label{fig:mitigation}
\end{figure*}

\iffalse
\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.32\textwidth]{Figures_Paper/FDI_DG4_mitigation_inputs.pdf}
        \label{fig:FDI_mitigation_input}
    } 
    \subfloat[]{
        \includegraphics[width=0.32\linewidth]{Figures_Paper/jamming_DG4_mitigation_inputs.pdf}
        \label{fig:jamming_mitigation_input}
    } 
    \subfloat[]{
        \includegraphics[width=0.32\linewidth]{Figures_Paper/sinusoidal_normal_DG4_mitigation_inputs.pdf}
        \label{fig:sinusoidal_mitigation_input}
    } \\ 
    
\caption[CR]{Detection and mitigation strategy applied at DG 4 under a random attack vector: (\subref{fig:FDI_mitigation}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage} attack against DGs 1 and 4, (\subref{fig:jamming_mitigation}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage} attack against DGs 1 and 4, (\subref{fig:sinusoidal_mitigation}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage} attack against DGs 1 and 4.} 
%\vspace{-2mm}
\label{fig:mitigation_inputs_random_attack_vector}
\end{figure*}
\fi




Fig.~\ref{fig:FDI_mitigation} shows the results of the mitigation strategy under the attack scenario of Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage}. The DG output voltage magnitude experiences a peak at $0.4s$, triggering the mitigation strategy with this sudden increase in the residual error. { The mitigation strategy is applied to DG 1 and 4. Hence, the voltages of the MG will try to synchronize with the reference value of 1 p.u. This action will make DGs 2 and 3 behave as if there were no attacks.} Fig. \ref{fig:jamming_mitigation} shows the mitigation action against the jamming attack scenario of Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage}. 
 {As shown in Fig. \ref{fig:jamming_attack_DG4}, Eq.  \eqref{eq:jamming-voltage} leads to higher perturbation at the output voltage of the DG. The detection and mitigation strategy leads to a slight voltage overshoot, increasing the effectiveness of the residual technique.} The results for the hybrid scenario of Eqs. \eqref{eq:hybrid-omega}, \eqref{eq:hybrid-voltage} are very similar, thus not reported for brevity.
Finally, Fig. \ref{fig:sinusoidal_mitigation} presents the mitigation action against the sinusoidal attack of Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage}. 
%Figures \ref{fig25} (a) and (b) deliberate on how the MG is dealing with a sinusoidal attack whenever a mitigation strategy is implemented. As far as we know, the L1 and ${l}^2$ norms of the residual error diverge in this type of situation. Due to the fact the sinusoidal function is introduced to our system, the behavior will not be linear. The same happened with the DoS attack. Those scenarios affect references of the output of the secondary controller. 
As seen in Fig. \ref{fig:sinusoidal_mitigation}, the internal voltage controller recovers the nominal reference value after $0.5s$ from the initialization of the attack. After mitigation is implemented, the effect on the frequency for all of the presented scenarios can be considered negligible. The demonstrated results confirm that the mitigation strategy effectively counters the impact of the attacks. The disruption observed after the attack onset depends on the detection threshold value. Small values could lead to false positives in the detection because of the presence of disturbances and noise in the system. On the other hand, high threshold values would considerably delay the mitigation's detection and activation. 



\iffalse

\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/Volt_freq_mit_stealthy_b_0.2.pdf}
        \label{fig:mitigation_stealthy_volt_0.2}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/Volt_freq_mit_stealthy_b_0.3.pdf}
        \label{fig:mitigation_stealthy_volt_0.3}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/Volt_freq_mit_stealthy_intermittent_b_0.2.pdf}
        \label{fig:mitigation_stealthy_interm_volt_0.2}
    } 
   \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/Volt_freq_mit_stealthy_intermittent_b_0.3.pdf}
        \label{fig:mitigation_stealthy_intermit_volt_0.3}
    } \\
    
    
\caption[CR]{Detection and mitigation strategy applied at DG 4 under a stealthy and intermittent attack with different b values: (\subref{fig:FDI_attack_DG4_INPUTS}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage}, (\subref{fig:JAMMING_attack_DG4_INPUTS}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage}, (\subref{fig:SINUSOIDAL_attack_DG4_INPUTS}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage}} 
\vspace{-3mm}
\label{fig: mitigation_inputs_stealthy_attack_vector}
\end{figure*}

\fi 
\iffalse
\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.315\textwidth]{Figures_Paper/Residual_FDI_Simple_Observer.pdf}
        \label{fig:FDI_L2norm_simple_obs}
    } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/Residual_JAMMING_Simple_Observer.pdf}
        \label{fig:Jamming_L2norm_simple_obs}
    } 
    % \subfloat[]{
    %     \includegraphics[width=0.2\linewidth]{Figures_Paper/L2norm_Sinusoidal_DG1_DG4.pdf}
    %     \label{fig:control1}
    % } 
    \subfloat[]{
        \includegraphics[width=0.315\linewidth]{Figures_Paper/Residual_Sinusoidal_Simple_Observer.pdf}
        \label{fig:sinusoidal_L2norm_simple_obs}
    } \\
    
\caption[CR]{${l}^2$ norm of the residual under random attack vectors using the Output Injection Observer approach: (\subref{fig:FDI_L2norm_simple_obs}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage} attack targeting DG 4, (\subref{fig:Jamming_L2norm_simple_obs}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage} attack targeting DG 4, (\subref{fig:sinusoidal_L2norm_simple_obs}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage} attack targeting DG 4.} 
%\vspace{-2mm}
\label{fig:l2norm_random_attack_simple_obs}
\end{figure*}



\begin{figure*}[t]
\centering
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/residual_stealthy_b_02_simple_observer.pdf}
        \label{fig:residual_stealthy_0.2_simple_observer}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/residual_stealthy_b_03_simple_observer.pdf}
        \label{fig:residual_stealthy_0.3_simple_observer}
    } 
    \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/residual_intermittent_b_02_simple_observer.pdf}
        \label{fig:residual_stealthy_intermittent_0.2_simple_observer}
    } 
   \subfloat[]{
        \includegraphics[width=0.23\linewidth]{Figures_Paper/residual_intermittent_b_03_simpleobserver.pdf}
        \label{fig:residual_stealthy_intermittent_0.3_simple_observer}
    } \\
    
\caption[CR]{${l}^2$ norm of the residual of DG4 under a stealthy and intermittent attack vector with different b values using the Output Injection Observer approach: (\subref{fig:residual_stealthy_0.2_simple_observer}) Eqs. \eqref{eq:fdia-omega}, \eqref{eq:fdia-voltage}, (\subref{fig:residual_stealthy_0.3_simple_observer}) Eqs. \eqref{eq:jamming-omega}, \eqref{eq:jamming-voltage}, (\subref{fig:residual_stealthy_intermittent_0.2_simple_observer}) Eqs. \eqref{eq:sinusoidal-omega}, \eqref{eq:sinusoidal-voltage}} 
\vspace{-3mm}
\label{fig: residuals_inputs_stealthy_attack_vector_simple_obs}
\end{figure*}
\fi
